Designing for Democratization: Introducing Novices to Artificial Intelligence Via Maker Kits

Existing research highlight the myriad of benefits realized when technology is sufficiently democratized and made accessible to non-technical or novice users. However, democratizing complex technologies such as artificial intelligence (AI) remains hard. In this work, we draw on theoretical underpinnings from the democratization of innovation, in exploring the design of maker kits that help introduce novice users to complex technologies. We report on our work designing TJBot: an open source cardboard robot that can be programmed using pre-built AI services. We highlight principles we adopted in this process (approachable design, simplicity, extensibility and accessibility), insights we learned from showing the kit at workshops (66 participants) and how users interacted with the project on GitHub over a 12-month period (Nov 2016 - Nov 2017). We find that the project succeeds in attracting novice users (40% of users who forked the project are new to GitHub) and a variety of demographics are interested in prototyping use cases such as home automation, task delegation, teaching and learning.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
		Corrected the bug with acmPrice.
		Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
		The package now is compatible with polyglossia (Joachim Breitner).
		Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

==> system.tex <==
\section{The System}
\begin{figure}
  \caption{Node.js code snippet shows how to prototype a voice command interaction using the TJBot library api. \label{fig:sampletjbotcode}}
\begin{lstlisting}
// Instantiate tjbotlib library
var tj = new tjbot(["microphone", "speaker","led","camera"], {}, credentials);
// Transcribe audio using Speech-to-Text AI service
tj.listen(function(msg) {
    if( msg.toLowerCase() == "what do you see" ){
        //Process camera image to Computer Vision AI service
        tj.see().then(function(objects){
            description = "Objects I see are "
            objects.forEach(function(object){
                description = description + " " + object
            }) // Synthesize audio using Text-to-Speech AI service, play using speaker
            tj.speak(description)
            // Change LED light to green.
            tj.shine("green")
        })
    }
})
\end{lstlisting}
\end{figure}

\subsection{Hardware}
The external body of TJBot is built from laser-cut chipboard parts which can also be 3D printed (see Figure \ref{fig:kitcomponents}, Figure \ref{fig:visualizationsnapshot}). The main electronic component is a Raspberry Pi hardware board[67] - an affordable yet functional credit-card sized computer that has become popular within the maker community for prototyping applications. The Pi is extensible and allows for the addition and control of multiple sensors and actuators via its (GPIO).  The kit also contains the following components as labeled in Figure \ref{fig:kitcomponents}: (part 11) Addressable RGB LED light that can be used to represent the state of the bot and can be programmed to reflect the entire range of RGB color codes. (part 10) A USB microphone that allows the recording of speech which can then be transcribed and processed to understand commands. (part 16) Servo motor installed in the arm of the robot that allows for mechanical control of the robot's arm. (part 12) Speaker box with support for both 3.5mm audio connection and Bluetooth (part 3) Camera (8 megapixels). Given that a primary focus of this work is designing to democratize AI services as opposed to robotics, the kit contains only a single mechanical piece.

\subsection{Software}
We selected JavaScript as the main programming language for TJBot given its ease of use and wide adoption \cite{Meyerovich2013EmpiricalAdoption,Stackoverflow} by various developers. Specifically, we use Node.js, an open-source cross-platform run-time environment that supports server-side JavaScript development. The Node.js architecture is expressive, functional without sacrificing performance \cite{Lei2014PerformanceJs,Tilkov2010Node.Programs} and has a vibrant, community-maintained repository of 3rd party libraries.
Programming TJBot entails 3 simple steps. First the user updates the operating system and their Node.js installation. Next, they create credentials that allow them access and integrate the cloud hosted services they are interested in prototyping with. They can then choose to download the sample code we provide from GitHub or write their own. We also provided a software library in Nodejs (TJBotlib) which encapsulates many functions for programming the kit into concise methods. To exemplify this, the code sample shown in Figure \ref{fig:sampletjbotcode} contains a program that allows the robot to respond to the question "what do you see?". Its response includes a spoken description of the scene and changing its LED light to green. Encapsulated functions within TJBotlib allows the user condense requests to multiple AI services (Speech to Text, Text to Speech, Computer Vision) and control kit hardware (microphone, speaker, camera and led) in 13 lines of code.
To further scaffold the learning experience and support a learning-by-doing approach we developed and published 3 sample code apps on GitHub that show how to (i) Control the LED on the robot using voice commands (ii) Allow the robot to connect to a live social media stream around a keyword and change its LED color based on recognized sentiment (iii) Design voice-based multi-turn conversations.

\subsection{Disseminating the Project}
To ensure the project was accessible to all users, we launched the project as an open source project by posting sample code and design files for the kit (laser cut and 3D print versions) on GitHub, providing detailed instructions on how to assemble the kit using the Instructables platform and sharing links to these resources on on social media (Twitter). GitHub was chosen because it is widely known, has a rich set of collaboration tools, and has an active community of developers. Instructables, was selected to host the instructional material we developed for the project given it is one of the largest online maker communities (over 29 million active users and over 100,000 projects ), and adopts a step-by-step presentation of instructions. Finally, we shared a blog post on the project on Twitter and encouraged users to share any projects they were conducting with the TJBot using the \#tjbot hashtag. 

